On the Feasibility of Reasoning about the Internal States of Blackbox IoT Devices Using Side-Channel Information

Internet of Things (IoT) devices are typically designed to function in a secure, closed environment, making it difficult for users to comprehend devices' behaviors. This paper shows that a user can leverage side-channel information to reason fine-grained internal states of black box IoT devices. The key enablers for our design are a multi-model sensing technique that fuses power consumption, network traffic, and radio emanations and an annotation interface that helps users form mental models of a black box IoT system. We built a prototype of our design and evaluated the prototype with open-source IoT devices and black-box commercial devices. Our experiments show a false positive rate of 1.44% for open-source IoT devices' state probing, and our participants take an average of 19.8 minutes to reason the internal states of black-box IoT devices.

==> ubicomp_parts/p2-threat.tex <==
\section{Threat Model}


We consider IoT devices to be trustworthy when we purchase them from the market. However, as we deploy them in our homes or offices, they may be hacked due to the cyber threat~\cite{shah2020survey}. For example, the attacker can remotely inject Trojans into the smart speaker to turn it into an eavesdropper~\cite{sidhu2019hardware}. The attacker can also leverage the laser to control the smart speaker~\cite{sugawara2019lightcommands}. There are ultrasound-based attacks to trigger the smart speakers to be vulnerable~\cite{roy2018inaudible}.  Therefore, it is essential to probe the IoT device's state after it is deployed in our homes or offices. We make the following assumptions about our adversarial model:
\begin{itemize}
    \item The IoT device that we purchase from the market is trustworthy, but it needs to be audited extensively to reveal all its normal states.
    \item With the proliferation of the cyber threat and ubiquitous internet connectivity, the attacker can easily conduct an attack to hack the IoT device deployed in our homes or offices.
    \item The attacker can stealthily and remotely hack the IoT device, triggering the IoT device to enter abnormal states. For example, the camera is on for spying while the light indicator is off. 
\end{itemize}













 


%As a result, individual electronic components generate consistent spikes (i.e., frequencies with strong signal strength) in the electromagnetic spectrum, since these frequencies correlate with the clock frequencies. 
%Further, since the current amplitude varies across different states, these circuits generate emanations with a characteristic signal strength distribution across a set of frequencies. 

% The most important emanation source is the clock signals since most electronic devices need clock signals to synchronize the circuit at the given frequency.
% The system's computing activities further modulate the clock signals' amplitude. 


% , which is usually a non-ideal square wave that will present many harmonics at multiples of the fundamental harmonics. 

% These emanations then propagate inside and outside the circuit, which is highly dependent on the characteristics of emanations in the frequency domain. 
% The time-domain emanations ideally should be a periodic square signal, This is because the clock signal is one of the most important sources for emanations, which is amplitude modulated by the computing activities of the system. Since the time-domain square wave is amplitude modulated, the emanations in the frequency domain will spread over the spectrum. Specifically, the Fourier transform of a periodic signal consists of a fundamental frequency and several harmonics at the multiples of the fundamental frequency. The sharper changes in the time-domain square wave, the higher frequencies of the harmonics.


% These emanations will propagate inside and outside the circuit. Therefore, these electromagnetic waves will be everywhere inside the circuit. 

% Some amplitude-modulated clock signals may excite the resonance of some modules (e.g., data lines) on the circuit. These data lines will act as antennas to radiate the emanations over the air outside the circuit. Moreover, the electronic device usually has RF transceivers,  such that these emanations can be mixed (i.e., due to an RF mixer), amplified (i.e., due to an amplifier), and broadcast through the transceiver's antennas over the air outside the circuit. 


% Power will propagate inside the circuit. 






% These variations will be correlated with the logic data (i.e., 0 and 1 values) processed by the system. 
% , leading to repetitive spikes in the EM spectrum. 

% periodic activity, such as that
% due to instruction loops, cause periodic variations in CPU
% power (i.e., sequence of DIVs followed by ADDs) that manifest as visible spikes in the EM spectrum

% Particularly, 

% Since these variations are the unintended results of the digital circuit's normal operation, we term them as emanations. 






